A Curiously Effective Backtracking Strategy for Connection Tableaux

Automated proof search with connection tableaux, such as implemented by Otten's leanCoP prover, depends on backtracking for completeness. Otten's restricted backtracking strategy loses completeness, yet for many problems, it significantly reduces the time required to find a proof. I introduce a new, less restricted backtracking strategy based on the notion of exclusive cuts. I implement the strategy in a new prover called meanCoP and show that it greatly improves upon the previous best strategy in leanCoP.

==> prftree/clausal-calc-ex.tex <==
\begin{prfenv}
{\prftree[r]{S}
{\prftree[r]{E (1.1)}
  {\prftree[r]{E (1.2)}
    {\prfbyaxiom{A}
    {\{\}, M, \{\mathsf{p}(x), \mathsf{r}(y)\}}}
    %
    {\prfbyaxiom{A}
    {\{\}, M, \{\mathsf{p}(x)\}}}
  {\{\mathsf{r}(y)\}, M, \{\mathsf{p}(x)\}}}
  %
  {\prfsummary{\text{\Lightning}}
  {\{\mathsf{q}(x)\}, M, \{\}}}
{{\{\mathsf{p}(x), \mathsf{q}(x)\}, M, \{\}}}}
{\varepsilon, M, \varepsilon}}
\end{prfenv}


==> prftree/clausal-calculus.tex <==
% Vertical alignment as explained in:
% https://tex.stackexchange.com/questions/7219/how-to-vertically-center-two-images-next-to-each-other/7222#7222

\newcommand\extensioninf{
  \begin{prfenv}
    \prftree[r]{E}
    {\prfassumption{C_2 \setminus \{L'\}, M, Path \cup \{L\}}}
    {\prfassumption{C                   , M, Path}}
    {C \cup \{L\}, M, Path}
  \end{prfenv}
}
\newcommand\extensioncond{
  where
    $C_2$ is a copy of $C_1 \in M$ and
    $L' \in C_2$ with $\sigma(L) = \sigma(\overline{L'})$
}

\input{prftree/common-calculus}
\renewcommand{\arraystretch}{2}
\begin{tabular}{m{\widthof{Reduction}} m{0.75\linewidth}}
  Axiom & \raisebox{-0.5\height}{\axiominf} \\
  Start & \calculusrule{\startinf}{\startcond} \\
  Reduction & \calculusrule{\reductioninf}{\reductioncond} \\
  Extension & \raisebox{-0.5\height}{\extensioninf} \\[-0.5em]
            & \extensioncond
\end{tabular}


==> prftree/common-calculus.tex <==
\newcommand\calculusrule[2]{
  \raisebox{-0.5\height}{#1}\raisebox{-0.5\height}{#2}
}

\newcommand\axiominf{
  \begin{prfenv}
    \prftree[r]{A}
    {}
    {\{\}, M, Path}
  \end{prfenv}
}

\newcommand\startinf{
  \begin{prfenv}
    \prftree[r]{S}
    {\prfassumption{C_2, M, \{\}}}
    {\varepsilon, M, \varepsilon}
  \end{prfenv}
}
\newcommand\startcond{
  where $C_2$ is a copy of ${C_1 \in M}$
}

\newcommand\reductioninf{
  \begin{prfenv}
    \prftree[r]{R}
    {C           , M, Path \cup \{L'\}}
    {C \cup \{L\}, M, Path \cup \{L'\}}
  \end{prfenv}
}
\newcommand\reductioncond{
  where $\sigma(L) = \sigma(\overline{L'})$
}


==> tikz/cutextdeep.tex <==
\begin{forest}
  for tree={cut},
  [
    [?,edge label={node[midway,xshift=0.1cm] {\Large \Leftscissors}}]
    [E,
      [?, name=right]
      [?, name=left]
    ]
  ]
  \path (left) -- node {\dots} (right);
  \draw[dotted] ($(left.west)-(0,3.9mm)$) to ($(right.east)-(0,3.9mm)$);
  \node at ($(right.east)-(-1mm,4mm)$) {\Large \Leftscissors};
\end{forest}



==> tikz/cutextshallow.tex <==
\begin{forest}
  for tree={cut},
  [
    [?]
    [E,
      [?, name=right]
      [?, name=left]
    ]
  ]
  \path (left) -- node {\dots} (right);
  \draw[dotted] ($(left.west)-(0,3.9mm)$) to ($(right.east)-(0,3.9mm)$);
  \node at ($(right.east)-(-1mm,4mm)$) {\Large \Leftscissors};
\end{forest}



==> tikz/cutred.tex <==
\begin{forest}
  for tree={cut},
  [
    [?,edge label={node[midway,xshift=0.1cm] {\Large \Leftscissors}}]
    [R]
  ]
\end{forest}



==> tikz/cuts.tex <==
\forestset{
  cut/.style={
    grow=north,
    draw, circle, inner sep=0.5mm,
    s sep=7mm,
    l sep=5mm,
    if={level() > 0}{minimum size=3mm}{}
  }
}
\subcaptionbox{Reduction (R).\label{fig:cutred}}[.25\linewidth]
{\input{tikz/cutred.tex}}
\subcaptionbox{Extension, inclusive (EI).\label{fig:cutextinclusive}}[.35\linewidth]
{\input{tikz/cutextdeep.tex}}
\subcaptionbox{Extension, exclusive (EX).\label{fig:cutextexclusive}}[.35\linewidth]
{\input{tikz/cutextshallow.tex}}


==> tikz/deepcut.tex <==
\begin{forest}
  for tree={
    grow=north,
    draw, inner sep=0.5mm,
    s sep=10mm,
    if={isodd(level)}{circle}{edge=dashed, rectangle}
  },
  [, name=root
    [, name=qX
      [, name=Xb]
    ]
    [, name=pX
      [, name=pXr]
      [
        [, name=rX
          [, name=Xar]
          [, name=Xal]
        ]
      ]
    ]
  ]
  \draw[->,dotted] (root) to[bend angle=45, bend left] node[left] {1} (Xal);
  \draw[->,dotted] (Xal) to[bend angle=15, bend left] node[above] {2} (qX);
  \node[right=0cm of qX] {3 \Lightning};
\end{forest}


==> tikz/generic.tex <==
\begin{forest}
  for tree={
    grow=north,
    draw, inner sep=0.5mm,
    s sep=10mm,
    if={isodd(level)}{circle}{edge=dashed, rectangle}
  },
  [
    [, edge label={node [midway, right] {$q(X)$}}
      [$C_6$, edge label={node [midway, right] {$X \mapsto b$}}]
    ]
    [, edge label={node [midway,  left] {$p(X)$}}
      [$C_3$]
      [$C_2$
        [, edge label={node [midway, left] {$r(X)$}}
          [$C_5$, edge label={node [midway, right] {$X \mapsto a$}}]
          [$C_4$, edge label={node [midway, left ] {$X \mapsto a$}}]
        ]
      ]
    ]
  ]
\end{forest}


==> tikz/nocut.tex <==
\begin{forest}
  for tree={
    grow=north,
    draw, inner sep=0.5mm,
    s sep=10mm,
    if={isodd(level)}{circle}{edge=dashed, rectangle}
  },
  [, name=root
    [, name=qX
      [, name=Xb]
    ]
    [, name=pX
      [, name=pXr]
      [
        [, name=rX
          [, name=Xar]
          [, name=Xal]
        ]
      ]
    ]
  ]
  \draw[->,dotted] (root) to[bend angle=45, bend left] node[left] {1} (Xal);
  \draw[->,dotted] (Xal) to[bend angle=15, bend left] node[above, very near start] {2} (qX);
  \draw[->,dotted] (qX) to[bend angle=60, bend left] node[below, near start] {3} (Xar);
  \draw[->,dotted] (Xar) to[bend angle=15, bend left] node[right, near start] {4} (pXr);
  \draw[->,dotted] (pXr) to[bend angle=45, bend left] node[above, near end] {5} (Xb);
\end{forest}


==> tikz/plot.tex <==
\centering
\begin{tikzpicture}
\begin{axis}
[ legend pos=south east
, xlabel=Time
, x unit=s
, ylabel=Problems solved
, no markers
, xmax=10
]
\addplot+ [solid] table {data/vampire-4.0-casc.integrated};
\addlegendentry{Vampire};
\addplot+ [dashed] table {data/bushy-meancop--conj--cutsrex};
\addlegendentry{meanCoP-REX};
\addplot+ [dashdotted] table {data/bushy-meancop--conj--cutsrei};
\addlegendentry{meanCoP-REI};
\addplot+ [densely dotted] table {data/plleancop-171116-sched.integrated};
\addlegendentry{leanCoP};
\addplot+ [dotted] table {data/plleancop-171116-nodef-cut-conj.integrated};
\addlegendentry{leanCoP-REI};
\end{axis}
\end{tikzpicture}


==> tikz/search.tex <==
\[\tag{1}
\left[
  \left[\begin{matrix}\tikzmarknode{m1p}{\mathsf{p}(x)} \\ \tikzmarknode{m1q}{\mathsf{q}(x)}\end{matrix}\right]
  \left[\begin{matrix}\tikzmarknode{m1np1}{\lnot \mathsf{p}(y)} \\ \tikzmarknode{m1r}{\mathsf{r}(y)}\end{matrix}\right]
  {\color{gray}\left[\begin{matrix}\lnot \mathsf{p}(z)\end{matrix}\right]}
  \left[\begin{matrix}\tikzmarknode{m1nr1}{\lnot \mathsf{r}(\mathsf{a})}\end{matrix}\right]
  {\color{gray}\left[\begin{matrix}\lnot \mathsf{r}(\mathsf{b})\end{matrix}\right]}
  {\color{gray}\left[\begin{matrix}\lnot \mathsf{q}(\mathsf{c})\end{matrix}\right]}
\right]\]
\begin{tikzpicture}[overlay,remember picture]
  \draw[->] (m1p.north) to [bend left] node [above] {1} (m1np1.north);
  \draw[->] (m1r.south) to [bend angle=30,bend right] node [above] {2} (m1nr1.south);
  \node[below] at (m1q.south) {\Lightning\,3};
\end{tikzpicture}

\[\tag{2}
\left[
  \left[\begin{matrix}\tikzmarknode{m2p}{\mathsf{p}(x)} \\ \tikzmarknode{m2q}{\mathsf{q}(x)}\end{matrix}\right]
  \left[\begin{matrix}\tikzmarknode{m2np1}{\lnot \mathsf{p}(y)} \\ \tikzmarknode{m2r}{\mathsf{r}(y)}\end{matrix}\right]
  {\color{gray}\left[\begin{matrix}\lnot \mathsf{p}(z)\end{matrix}\right]}
  {\color{gray}\left[\begin{matrix}\lnot \mathsf{r}(\mathsf{a})\end{matrix}\right]}
  \left[\begin{matrix}\tikzmarknode{m2nr2}{\lnot \mathsf{r}(\mathsf{b})}\end{matrix}\right]
  {\color{gray}\left[\begin{matrix}\lnot \mathsf{q}(\mathsf{c})\end{matrix}\right]}
\right]\]
\begin{tikzpicture}[overlay,remember picture]
  \draw[->] (m2p.north) to [bend left] (m2np1.north);
  \draw[->] (m2r.south) to [bend angle=25,bend right] node [above] {1} (m2nr2.south);
  \node[below] at (m2q.south) {\Lightning\,2};
\end{tikzpicture}

\[\tag{3}
\left[
  \left[\begin{matrix}\tikzmarknode{m3p}{\mathsf{p}(x)} \\ \tikzmarknode{m3q}{\mathsf{q}(x)}\end{matrix}\right]
  {\color{gray}\left[\begin{matrix}\lnot \mathsf{p}(y) \\ \mathsf{r}(y)\end{matrix}\right]}
  \left[\begin{matrix}\tikzmarknode{m3np2}{\lnot \mathsf{p}(z)}\end{matrix}\right]
  {\color{gray}\left[\begin{matrix}\lnot \mathsf{r}(\mathsf{a})\end{matrix}\right]}
  {\color{gray}\left[\begin{matrix}\tikzmarknode{m3nr2}{\lnot \mathsf{r}(\mathsf{b})}\end{matrix}\right]}
  \left[\begin{matrix}\tikzmarknode{m3nq}{\lnot \mathsf{q}(\mathsf{c})}\end{matrix}\right]
\right]\]
\begin{tikzpicture}[overlay,remember picture]
  \draw[->] (m3p.north) to [bend left] node [above,very near end] {1} (m3np2.north);
  \draw[->] (m3q.south) to [bend angle=17,bend right] node [above] {2} (m3nq.south);
\end{tikzpicture}


==> tikz/shallowcut.tex <==
\begin{forest}
  for tree={
    grow=north,
    draw, inner sep=0.5mm,
    s sep=10mm,
    if={isodd(level)}{circle}{edge=dashed, rectangle}
  },
  [, name=root
    [, name=qX
      [, name=Xb]
    ]
    [, name=pX
      [, name=pXr]
      [
        [, name=rX
          [, name=Xar]
          [, name=Xal]
        ]
      ]
    ]
  ]
  \draw[->,dotted] (root) to[bend angle=45, bend left] node[left] {1} (Xal);
  \draw[->,dotted] (Xal) to[bend angle=15, bend left] node[above] {2} (qX);
  \draw[->,dotted] (qX) to[bend angle=15, bend left] node[below] {3} (pXr);
  \draw[->,dotted] (pXr) to[bend angle=15, bend left] node[above, near end] {4} (Xb);
\end{forest}


==> tikz/stack.tex <==
\centering
\subcaptionbox{No cut.\label{fig:nocut}}[.17\linewidth]
{
\begin{tikzpicture}
\draw (0,0) rectangle ++(1cm,8em);
\node at ($(0,0)!0.5!(1cm,1em)$) {$a_1$};
\node at ($(0,1em)!0.5!(1cm,4em)$) {$\vdots$};
\draw (0,4em) rectangle ++(1cm,1em) node[midway] {$a_n$};
\node at ($(0,5em)!0.5!(1cm,8em)$) {$\vdots$};
\end{tikzpicture}
}
\subcaptionbox{Exclusive.\label{fig:cutexclusive}}[.17\linewidth]
{
\begin{tikzpicture}
\draw (0,0) rectangle ++(1cm,5em);
\node at (.5cm,.5em) {$a_1$};
\node at (.5cm,2.75em) {$\vdots$};
\draw (0,4em) rectangle ++(1cm,1em) node[midway] {$a_n$};
\end{tikzpicture}
}
\subcaptionbox{Inclusive.\label{fig:cutinclusive}}[.2\linewidth]
{
\begin{tikzpicture}
\draw (0,0) rectangle ++(1cm,4em);
\node at (.5cm,.5em) {$a_1$};
\node at (.5cm,2.75em) {$\vdots$};
\end{tikzpicture}
}

